One Arrow, Two Kills: An Unified Framework for Achieving Optimal Regret Guarantees in Sleeping Bandits

We address the problem of \emph{`Internal Regret'} in \emph{Sleeping Bandits} in the fully adversarial setup, as well as draw connections between different existing notions of sleeping regrets in the multiarmed bandits (MAB) literature and consequently analyze the implications: Our first contribution is to propose the new notion of \emph{Internal Regret} for sleeping MAB. We then proposed an algorithm that yields sublinear regret in that measure, even for a completely adversarial sequence of losses and availabilities. We further show that a low sleeping internal regret always implies a low external regret, and as well as a low policy regret for iid sequence of losses. The main contribution of this work precisely lies in unifying different notions of existing regret in sleeping bandits and understand the implication of one to another. Finally, we also extend our results to the setting of \emph{Dueling Bandits} (DB)--a preference feedback variant of MAB, and proposed a reduction to MAB idea to design a low regret algorithm for sleeping dueling bandits with stochastic preferences and adversarial availabilities. The efficacy of our algorithms is justified through empirical evaluations.

==> res.tex <==
\section{Experiments}

\section{Conclusion and future work}

\iffalse%%%%%%%%%%%%%%%%%%%%%%%%%

\section*{Questions/Ideas}

\begin{itemize}[nosep]
    \item Battling bandit with more arms
    \item Improving the dependence on $K$
    \item Applying the result of Zimmert with OMD to achieve gap dependent bounds.
    \item Showing that sleeping internal regret implies ordering regret for i.i.d. availabilities.
    \item 
\end{itemize}


Now Pierre writing: Can we come up with an algorithm for low internal regret with sleeping bandits for MAB. Once we have the result for MAB, we can do the reduction idea to get the "low" internal regret algorithm for DB. 

We already show (Lem): 1. For stochastic losses and stoc sleeping,  "low" internal regret implies "low" ordering regret (as well as low policy regret)
 
 

Yet to solve:---

1. For stochastic sleeping and adversarial losses, does "low" internal regret implies "low" ordering regret ?

2. For stochastic sleeping and adversarial losses, (where losses/ rewards are chosen independent of the subset availabilities), does ordering regret (this paper) and policy regret (ICML20 paper) equivalent of the later is stronger?

3. 

Expts:

MAB: 3 algos) Klienberg (stoc rewards \& adv sleeping), ICML20 (other way), and our internal regret based algorithm

>> Settings: (a) Stoc rew and adv sleeping (b)  Adv rew and stoc sleeping

DB1: Compare Neurips paper vs our reduction+internal regret (for Stoc rew and adv sleeping)

DB2: Reduction+ICML20 --- Compare performance of DB1 with 

\fi%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
